Data-Driven Vulnerability Detection and Repair in Java Code

Java platform provides various APIs to facilitate secure coding. However, correctly using security APIs is usually challenging for developers who lack cybersecurity training. Prior work shows that many developers misuse security APIs; such misuses can introduce vulnerabilities into software, void security protections, and present security exploits to hackers. To eliminate such API-related vulnerabilities, this paper presents SEADER -- our new approach that detects and repairs security API misuses. Given an exemplar, insecure code snippet, and its secure counterpart, SEADER compares the snippets and conducts data dependence analysis to infer the security API misuse templates and corresponding fixing operations. Based on the inferred information, given a program, SEADER performs inter-procedural static analysis to search for any security API misuse and to propose customized fixing suggestions for those vulnerabilities. To evaluate SEADER, we applied it to 25 <insecure, secure> code pairs, and SEADER successfully inferred 18 unique API misuse templates and related fixes. With these vulnerability repair patterns, we further applied SEADER to 10 open-source projects that contain in total 32 known vulnerabilities. Our experiment shows that SEADER detected vulnerabilities with 100% precision, 84% recall, and 91% accuracy. Additionally, we applied SEADER to 100 Apache open-source projects and detected 988 vulnerabilities; SEADER always customized repair suggestions correctly. Based on SEADER's outputs, we filed 60 pull requests. Up till now, developers of 18 projects have offered positive feedbacks on SEADER's suggestions. Our results indicate that SEADER can effectively help developers detect and fix security API misuses. Whereas prior work either detects API misuses or suggests simple fixes, SEADER is the first tool to do both for nontrivial vulnerability repairs.

==> Approach/Drill.tex <==
\subsubsection{Drill SourceCodeChange}
When determining the type of \emph{CodePattern}, we need to dig into AST to get the information. However, ChangeDistiller does not indicate this type of information. Hence, we use two \emph{SourceCodeRange} to locate the original statement and traverse its AST to get more information.

Specifically, we use Eclipse AST framework~\cite{eclipse} in this step. We will use \emph{SourceCodeRange} from the last step to get the original step. Next, we call \emph{NodeFinder} to find the corresponding node (subtree) which represents our target statement. Then we will walk through this subtree to get information includes binding information and its parameter list. The algorithm is shown in Algorithm \ref{alg:pattern}.   

\begin{algorithm}
  \caption{Pattern Determined}
  \label{alg:pattern}
  \begin{algorithmic}[1]
    \Function {GetPattern}{}
        \State oldNode = Nodefinder.perform(OldsourceCodeRange)
        \State newNode = Nodefinder.perform(NewsourceCodeRange)
        \State Walk through oldNode and newNode Get binding information and parameter list
        \State Generate matching expression for oldNode and newNode
    \EndFunction
  \end{algorithmic}
\end{algorithm}

Note that we implemented our custom visitor that is extended from ASTVisitor. Since when traversing the ASTNode, ASTVisitor needs to implemented in eclipse AST. Besides, when we walk through the note, we will create a matching expression automatically for the statements. The matching expression will be based on the invocation method, binding information, and its parameter. For instance, given a statement: %\mint{java}
|Cipher c = Cipher.getInstance("AES");|, it will be transformed into the matching expression below:
%\mint{Java}
|Cipher.getInstance("\$sl");| The leading variable declaration will be discarded since it will not compromise secure. If the parameter is a numeric value, it will be transformed \emph{"\$nl"} which stands for number literal. 

After getting the matching expression and parameter list, the next step will be to determine the type of pattern. The condition of each pattern is listed below:
\begin{itemize}
    \item Parameter Pattern: The parameter is string literal.
    \item Number Pattern: The parameter is number literal, and it has a minimum secure threshold. 
    \item Name Pattern: The function name is different.
    \item Composite Pattern: There are multiple statements in the \emph{SourceCodeChange} list.
\end{itemize}

Note that if a method has multiple parameters, we will separate them into multiple matching expression and use an indicator to point out which parameter needs to be checked. For example, given a statement  %\mint{Java}
|cipher.init(Cipher.ENCRYPT\_MODE, key);|, and we want to check if the key is secure. In our matching expression, it will become: 
%\mint{Java}
|cipher.init(\$sl, Key); \#2| The following number will indicate the index of the parameter we need to check.

Another case is to handling slash ("/"). Since Java security framework only provides limited encryption algorithms\footnote{Available algorithms can be checked on \url{https://docs.oracle.com/javase/8/docs/technotes/guides/security/StandardNames
.html}}, some of them have the following pattern: ``algorithm/mode/padding".\footnote{https://docs.oracle.com/en/java/javase/12/docs/api/java.base/javax/crypto/
Cipher.html} To decrease the number of expression patterns, we introduce the wildcard symbol: ``\$". When detecting ``\$", our tool will skip this specific value. 

\subsubsection{Direct Generator}
Sometimes, developers will already have the parameter list that includes the insecure and secure cases. We create a tool that can read our template to obtain the insecure and secure parameters directly. The template is shown in Listing \ref{exp:temp}. We have some restrictions on the template so that our direct generator can handle it:
\begin{itemize}
    \item Template should be completed and executable.
    \item There should be two sets named \emph{insecure} and \emph{secure} and a variable \emph{pos} in the template. Variable names cannot be changed.
    \item After declaring two sets, a statement for generating matching expressions should follow. 
\end{itemize}
\begin{listing}
import javax.crypto.Cipher;
import java.util.Arrays;
import java.util.HashSet;
import java.util.Set;
public class test {
    public void main(String[] args) throws Exception{
        Set<String> insecure = 
        new HashSet<>(Arrays.asList("a"));
        Set<String> secure = 
        new HashSet<>(Arrays.asList("c"));
        Cipher c = Cipher.getInstance("AES");
        int pos = 0;
    }
}    
    \caption{Direct Generator Template}
    \label{exp:temp}
\end{listing}

The restrictions must be met since a) A incomplete code cannot generate binding information correctly. It will affect the success rate when detecting the error; b) The generator is written by rules; it cannot detect the content intelligently. If the rules cannot be satisfied, the generator will throw a runtime error.

For implementing the generator, we use JavaParser~\cite{hosseini2013javaparser} instead of Eclipse API since JavaParser provides some powerful API that can improve the readability of the code. Generator will first fetch insecure and secure parameters from these two sets and store it into \emph{iSet} (insecureSet) and \emph{cSet} (secureSet) respectively. Next, it will find \emph{pos} to get the index of parameter. Then, it will filter all statements in the file that belongs to \emph{methodCallExpr} class\footnote{The type of statements in JavaParser is slightly different from the one in Eclipse AST. Please refer to the document: https://www.javadoc.io/doc/com.github.javaparser/javaparser-core/3.14.1}. After filtering, there will be only one statement left which is the statement for the matching expression. We obtain binding information of this statement, build the matching expressions and save it to the database.

Note that the parameter in the target statement (Line 11, ``AES") will be ignored. The generator will treat that parameter as a placeholder and will not do any work on it. 

==> Approach/PatternGeneration.tex <==
% give a total overview of our design
% 1. overview, our design
% 2. Tools - changedistiller
% 3. four patterns and its representation

In this section, the overview of our approach will be given. Next, we describe how we utilize ChangeDistiller~\cite{fluri2007change} to get the change script. Then we dig into the change script to find the patterns and provide a direct generator tool. To reuse the pattern, we present two methods to store the patterns. For detecting the error, we show a backward slicing approach on target codes to get the relative code statement that can be matched to the code in our code database.  

\subsection{Overview}
As shown in Fig. 1, we will first use ChangeDistiller to compare corresponding insecure and secure code snippets. After ChangeDistiller returns the change script, we will categorize the change script into one pattern as shown in Fig \ref{fig:pattern}.  

In our approach, we implement an interface - CodePattern. In CodePattern, it defines the basic information about a pattern. Note that CodePattern is serializable which allows the patterns to be saved in files directly. There is four class inherited from CodePattern: Parameter Pattern, Number Pattern, Name Pattern, and Composite Pattern. If a parameter pattern exists, it means that we need to check the parameter to see if the code is secure. If it is a number pattern, we will check if the value within the parameter list in a function or the time of iterations is big enough to be secure. If it is a name pattern, the method needs to be changed from an insecure implementation to a secure one. And a composite pattern stands for multiple statements needs to be check. After finishing generating the pattern, we will persist the data and store to database. 
\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{codepattern.pdf}
    \caption{Pattern Categories}
    \label{fig:pattern}
\end{figure}

After having the patterns, we will detect the potential insecure statements in the target Jar files. We perform a backward slicing to a target statement to get the corresponding statements based on WALA~\cite{watsonwatson}. Then we compare with our existing data and give a suggestion to the developer about what kind of changes need to be made to make the code secure.

\subsection{Obtain the pattern by ChangeDistiller}
%introduce Changedistiller and its basic operations. How we can get the pattern from changedistiller. Analyze four patterns and the difference between them.
To get the code difference, we use ChangeDistiller in our work. ChangeDistiller is a tool that can extract source codes difference based on tree differencing. It takes two codes as input, transform them into two abstract syntax trees (AST) and compare the difference between them. Then it will return a script about how to make these two codes identical. The script is composed of operations which include insert, delete, update and move. For simplicity, the pair of insecure and secure codes we run in this step is pretty simple and neat. It means that we will remove any extra statement in our code which is shown in Fig. \ref{fig:codediff}. Hence, the operations will be limited to insert, delete and update. 

When ChangeDistiiler finishing generating the difference, it will return a list of \emph{SourceCodeChange}s. \emph{SourceCodeChange}s is a abstract interface. It is inherited by \emph{Insert}, \emph{Delete} and \emph{Update} Class as shown in Fig \ref{fig:sccDiagram}. Overall, they all have a member variable named SourceCodeRange which can be represented as \emph{[start, end]}. \emph{Start} is the character position of the beginning of the statement or how many characters before this statement. \emph{end} is the end character of this statement. For \emph{Insert}, it will return the position that we need to insert the statement while \emph{Delete} will return the position that we need to delete the statement. \emph{Update} will be complicated since it will return two \emph{SourceCodeRange}s which is for insecure file and secure file respectively. 
\begin{figure}[hbtp]
    \centering
    \includegraphics[width=0.45\textwidth]{class.pdf}
    \caption{SourceCodeChange UML Class Diagram}
    \label{fig:sccDiagram}
\end{figure}

\begin{figure*}[hbtp]
    \centering
    \includegraphics[width=\textwidth]{code_diff.png}
    \caption{Code Difference Example}
    \label{fig:codediff}
\end{figure*}

One will argue that \emph{Update} is not necessary since every update command can be decomposed as a combination of \emph{Insert} and \emph{Delete}. Note that when editing the code, we will direct manipulate AST not the actual code. \emph{Insert} and \emph{Delete} is more expensive than a \emph{Update} since removing a subtree and insert a new subtree is costlier than change the value directly to a subtree. Hence \emph{Update} will exist on our design.

However ChangeDistiller will return \emph{Update} command. But it is not enough for our analysis. When we get \emph{Update} command, we need to know what causing the difference such as parameters. In the next section, we will show an approach to dig more information from \emph{Update} command.





==> Approach/Persistance.tex <==
\subsection{Data Persistence}
After generating the pattern, the pattern should be saved properly so that it can be reused in the future. In our tool, we provide two options to save the patterns:
\begin{itemize}
    \item JSON File: All CodePattern will be saved into a single JSON file. When the detection runs, it will load the pattern to the memory. In the JSON file, we will store the type of code patterns, and the function SAFI should be checked. Excepted the common fields, we design different fields for each code patterns, which is listed at Table \ref{tab:JSON}:
    \begin{table}[hbtp]
    \centering
    \begin{tabular}{c|c|c}
        \hline
        Type & Field & Comment \\ 
        \hline
        \multirow{3}{*}{Parameter} & Check & The \#th of parameter need to be checked \\\cline{2-3} & Incorrect & Insecure parameters set \\ \cline{2-3} & Correct & Secure parameters set \\
        \hline
        \multirow{3}{*}{Number} & Check & The \#th of parameter need to be checked \\\cline{2-3} & MinNum & The minimum number should be met \\ \cline{2-3} & Correct & The suggestions  \\
        \hline
        Name & correct & the correct function should be used \\
        \hline
    \end{tabular}
    \caption{JSON structs}
    \label{tab:JSON}
\end{table}
    \item Database: For further data processing, SAFI also provides a database option to store the pattern. The struct of database tables is similar to the JSON file. 
\end{itemize}

==> Approach/VirnerabilityFix.tex <==
\subsection{Generate Fix Patch}

When detecting the error, SAFI will generate the fix patch by the type. As we mentioned in Figure~\ref{fig:pattern}, SAFI will triage the patterns into two major types: the composite pattern (parameter, type, and name) and non-composite pattern when generating the fix patch. 

\subsubsection{Non-composite Pattern}

For the non-composite pattern, SAFI will give suggestions based on the data in the database. The algorithm can be represented below: 
\begin{algorithm}
  \caption{Non-Composite Fix Generator}
  \label{alg:pattern}
  \begin{algorithmic}[1]
    \Function {NonCompositeFixGenerator}{p: CodePattern}
        \State Switch Type(CodePattern)
        \State \hskip1em Case "Parameter" -> Check Parameter and give fix
        \State \hskip1em Case "Name" -> Check function name and give fix
        \State \hskip1em Case "Number" -> Check if the parameter is lower than the number
    \EndFunction
  \end{algorithmic}
\end{algorithm}

For instance: 
%\mint{java}
|Cipher.getInstance("DES/ECB/PKCS5Padding")|
SAFI will first detect that \emph{Cipher.getInstance} is a parameter pattern, and it should check the first parameter of the function. Then SAFI will check if \emph{DES/ECB/PKCS5Padding} is in the incorrect set. If so, it will give several secure suggestions to users. The name and number pattern will follow these steps too. 

\subsubsection{Composite Pattern}
For the composite pattern, SAFI will first get all relative statements using the forward slicing. Then it will normalize all relative statements, and calculate the similarity with the correct template using normalized Levenshtein distance~\cite{yujian2007normalized}. The normalize Levenshtein Distance can be presented as:
\begin{equation*}
    S(s1,s2) = \frac{Levenshtein(s1, s2)}{\max(s1.len, s2.len)},
\end{equation*}
where s1 and s2 are two strings. If \emph{S} is greater than the threshold, SAFI will treat s1 and s2 as identical strings. Meanwhile, it will match the normalized variables. If SAFI finds missing statements, it will try to match the original context and give the suggestion to user to add the missing statement with the context. A working example is showed in Figure~\ref{fig:program}.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{multiline.pdf}
    \caption{Composite Pattern Example}
    \label{fig:program}
\end{figure}



==> Approach/slicingDetection.tex <==
\subsection{Detect the Vulnerability}
% Provide several examples about the importance using slicing.
% Give a brief introduction about slicing

According to the generated patterns, there is mainly two part of the vulnerability should be taken care, one it is the wrong parameter/API name selection; the other is the API invocation sequence problem. For parameter/API name selection, we implement the customized backward slicing to tracing the def-use chain step by step, which achieve both the intra-and inter- procedural analysis for Java project. For API Invocation sequence, we use the WALA built-in forward slicing to obtain the relative statements. 

\subsubsection{Def-Use Chain}

As  Figure \ref{fig:slicing}  shows,  if we want to analyze if there is some vulnerability on \emph{Cipher.getInstance}. We will determine if the \emph{used} variable \emph{algo} is a secure option. We need to trace back the \emph{def} line to retrieve the value of \emph{algo}. When facing the actual code, we cannot expect that the code is clean, like the code in our dataset. Therefore, we categorize the declaration of \emph{algo} into the following four scenarios:  

\textbf{Within\_Method. }  the \emph{def} could be traced within one method 

\textbf{Passin\_Parameter. } the \emph{def} could be in any other function, within or without the same class, the value of the variable \emph{algo} is passed as a parameter to the function which calls the target function  

\textbf{Field\_Declaration. } the \emph{def} is the static field or field declared in a class with value assigned

\textbf{Init\_Constructor. } the \emph{def} is the static field or field declared in a class, the value is assigned within a constructor.

\begin{figure}[hbtp]
    \centering
    \includegraphics[width=0.45\textwidth]{slicing.pdf}
    \caption{Backward Slicing Example on Listing \ref{exp:crypto}}
    \label{fig:slicing}
\end{figure}

\todo[inline]{need modify the backward slicing algorithm, add algorithm figue}
%Slicing is a technique which can prune the codes which is irrelevant to the target statement. For backward slicing, the algorithm will find all statements that might affect the state of the target statement. For example, in Fig.~\ref{fig:slicing}, the statement that will affect the result of \emph{Cipher.getInstance} is Line 3 which is the declaration of \emph{crypto}. Hence, when detecting the error, we will first do the backward slicing on security-related method calls, and check if they are secure. In our approach, we utilize WALA to perform backward slicing.
%eHowever, the actual backward slicing algorithm is sophisticated. It first transforms JAVA code into SSA IR~\cite{wala}, then performs backward slicing on system dependency graph~\cite{horwitz1988interprocedural}. 
\subsubsection{Backward Tracing Algorithm}
Slicing is a technique that can prune the codes, which is irrelevant to the target statement. For backward slicing, the algorithm will find all statements that might affect the state of the target statement. For example, in Fig.~\ref{fig:slicing}, the statement that will affect the result of \emph{Cipher.getInstance} is Line 3 which is the declaration of \emph{crypto}. Hence, when detecting the error, we will first do the backward slicing on security-related method calls, and check if they are secure. 

In our approach, we utilize WALA to perform backward slicing. It first transforms JAVA code into SSA IR~\cite{wala}, then performs backward slicing on the system dependency 
graph~\cite{horwitz1988interprocedural}.  However, the actual backward slicing algorithm directly returns the related statements while our target is the most recent \emph{def} value stored in the Symbol table.  In order to trace back the \emph{def-use} chain of the target variable,  we implement the backward tracing algorithm based on WALA BackwardSuperGraph~\cite{horwitz1988interprocedural}.  As Figure \ref{} shows, after locating the security-related API invocation, our algorithm first performs Intra-procedural analysis; it uses the \emph{def-use} number to construct a \emph{def-use} chain in the current method from the API invocation place. In each construction step, our algorithm will use the number mapping back to the \emph{SymbolTable} within current method, if the value could be retrieved, then it would compare with the value with the insecure dataset.
If the intra-procedural analysis can't retrieve corresponding \emph{def} the number for the target \emph{use},  our algorithm would further apply the inter-procedual backward tracing to locate the caller statement, determine the \emph{use} in which four of the category listed above, then interactively performance the process as intra-procedural analysis.

When WALA transforms JAVA code into SSA IR, it will optimize the actual code. For example, the Line 3 and Line 6 in Listing \ref{exp:crypto} will be combined into:     

   Cipher cipher = Cipher.getInstance("DES/ECB/PKCS5Padding");


Therefore, after backward slicing, WALA will return the result list which consists of statements. In the above case, there will be only one statement in the list. We iterate \emph{symboltable} in the IR which represents the statement to find the parameter. Besides, we obtain the function signature as binding information to match the data in the database. 

\subsubsection{Composite Patterns Detection}

Composite Patterns are the multiline scenarios and the trustmanager\footnote{\url{https://docs.oracle.com/en/java/javase/12/docs/api/java.base/javax/net/ssl/X509TrustManager.html}}. For the multiline scenarios, SAFI will use the forward slicing to retrieve all related statements. Then all variable names in the retrieved statements are replaced using the following rules:  ``\$v\_\textbackslash d+", which means the variable name started with ``\$v\_" and followed by a number. We will eleborate it in Section 3.5. 

A typical SSL code abstraction is shown at Listing~\ref{exp:ssl}. SAFI will check if \emph{checkClientTrusted} and \emph{checkServerTrusted} is empty and if these two functions throw any exceptions. 

\begin{lstlisting}
   
    void  checkClientTrusted  
        (X509Certificate[] chain, String authType) {}
    void. checkServerTrusted  
        (X509Certificate[] chain, String authType) {}
    X509Certificate[]  getAcceptedIssuers()
        \caption{TrustManager Abstraction}
    \label{exp:ssl}
\end{lstlisting}

==> Result/EvaluationDesign.tex <==
% question, related work, ruleset, extendsion. addtional rule. extendsion. example. flexible.  

\section{Evaluation}
This section describes the training data set and the performance of our tool on the test data set and the pattern we generated, and then we present our research questions (RQs) and its results. Finally, we discuss the limitation of the tools in the current implementation status. 

\subsection{Data Set}
\textbf{Training dataset} We use the data set crawled from StackOverflow, which related to cryptography API usage~\cite{chen2019reliable}; this dataset includes 785 secure answer posts and 644 insecure answer posts. We further 1) paired the insecurity code examples with the corresponding security codes; 2) pruned unrelated code to make each code example only includes one of the vulnerability; 3) constructed the code snippets to the compilable program and manually fixed the vulnerability code snippet if there is no matched security code snippet in the dataset. Since there are a lot of code snippets reflect the same API misuse case, we also removed the duplicated case. Overall, we have a training dataset which contains 72 pair of codes. Since the options for writing the insecure codes and secure codes are limited, the number of the training dataset is unnecessary to be large.

% \begin{listing*}
%     \begin{minted}[mathescape,
%                   linenos,
%                   breaklines,
%                   numbersep=5pt,
%                   gobble=0,
%                   fontsize=\small,
%                   frame=lines,
%                   framesep=2mm]{java}
% public class EcbInSymmCryptoABICase1 {
%     public void go(String crypto) throws NoSuchPaddingException, NoSuchAlgorithmException, InvalidKeyException {
%         KeyGenerator keyGen = KeyGenerator.getInstance("AES");
%         SecretKey key = keyGen.generateKey();
%         Cipher cipher = Cipher.getInstance(crypto);
%         cipher.init(Cipher.ENCRYPT_MODE, key);
%     }

%     public static void main (String [] args) throws NoSuchPaddingException, NoSuchAlgorithmException, InvalidKeyException {
%         EcbInSymmCryptoABICase1 bc = new EcbInSymmCryptoABICase1();
%         String crypto = "AES/ECB/PKCS5Padding";
%         bc.go(crypto);
%     }
% }
%     \end{minted}
%     \caption{The Code Causing Wrong Parameter Retrieval}
%     \label{exp:wrong}
% \end{listing*}


==> Result/EvaluationPattern.tex <==
\subsection{Pattern Generation}
Before we compare to state-of-the-art, we first use our train dataset to generate the template for detection. For each pair of the code, this tool generates the API misuse pattern by analyzing the code difference. It extracts the binding information for invoked API, records the API name with incorrect usage format, and the fixed operation. This tool generates 13 patterns from the training dataset. We categorized these pattern into Four different part:  

\textbf{Parameter pattern:} This pattern related to the encryption algorithm misuse within a method invocation. The incorrect and correct usage of algorithms could be enumerated and the fixed method is updating the algorithm with the correct one.

\textbf{Number pattern:} This pattern related to incorrect usage of number value range such as key size.  Compared with parameter pattern, this pattern should reflect the incorrect value range information, so when fixing such vulnerabilities, we need to compare the value range information and picked a security value.  

\textbf{Name Pattern:} This pattern related to the API name replacement. 

\textbf{Composite pattern:} This pattern includes a block of the code statements replaced with another block of the statements. For example, a static declared password should be replaced with a randomly generated password. 

% \todo[inline]{one rule, one categories. multi-line, vulnerability, comparision with other tools}

The generated pattern is shown in Table~\ref{tab:Pattern}. When checking the parameter and number, SAFI will also generate the index of arguments need to be checked. 

\begin{table}[hbtp]
    \centering
    \begin{tabular}{c|c}
        Pattern Type & Inspection Function\\
        \hline
        \multirow{8}{*}{Parameter} & Cipher.getInstance\#0 \\& MessageDigest.getInstance\#0 \\ & SSLContext.getInstance\#0 \\ & SecretKeySpec.<init>\#0 \\ & SecureRandom.setSeed\#0 \\ & IvParameterSpec.<init>\#0 \\ & PBEKeySpec.<init>\#0 \\ & PBEKeySpec.<init>\#1 \\
        \hline
        \multirow{2}{*}{Number} & KeyPairGenerator.initialize \\ & PBEKeySpec.<init>\#2 \\
        \hline
        Name & Random.<init> \\
        \hline
        \multirow{2}{*}{Composite Pattern} & Trust Manager \\ & HostnameVerifier \\
        \hline
    \end{tabular}
    \caption{Pattern Generation}
    \label{tab:Pattern}
\end{table}




==> Result/EvaluationRQ1.tex <==
%   1. comparsion how tool work compare state art, ,comparesion dataset,performace. time performace. include the time. based on 13 project. precision, recall. time, work. comparsion. introduce. 
\subsection{RQ1: How does the detection of SAFI compare to the state-of-the-art?}

We evaluate our tool and the state-of-the-art in the following dimensions:
\begin{itemize}
    \item Running Time: the execution time of tool to generate the result.
    \item Precision: the correctness of the result.
    \item Recall: \textcolor{red}{123}
    \item Configuration: How easy to add a new pattern.
\end{itemize}

To verify the correctness of detection, we choose CryptoAPI \footnote{\url{https://github.com/CryptoGuardOSS/cryptoapi-bench/tree/master/src/main/java/org/cryptoapi/bench}}, which includes 197 programs that covers 14 kinds of API misuse and 13 jar files which are from 100 open-source projects. The experiment result is shown at Table~\ref{tab:cryptoBench}, ~\ref{tab:Apache Running Time} and~\ref{tab:Apache Result}. 

The CryptoAPI is for testing the coverage of SAFI generated pattern template. In CryptoBench, it contains various methods of calling crypto API such as inter-procedural and intra-procedural call. It helps to examine if the detection tool can handle the common code usage in practical. As shown in Table~\ref{tab:cryptoBench}, we pass all 14 kinds of API misuses. Meanwhile, we manually review all the given fix. It all fits the original code context and can be compiled. 

Table~\ref{tab:Apache Running Time} and Table~\ref{tab:Apache Result} is for comparing the accuracy and the running time between SAFI and CryptoGuard against the practical projects.
For human inspection, we ask a student who has experience in security API and provides him a checklist. In general, SAFI can generate the result closer to human inspection and runs faster than the CryptoGuard. Note that human inspection might miss some cases, and it cannot be treated as ground truth. From Table~\ref{tab:Apache Result}, we conclude that 1) SAFI can find out more cases than humans; 2) SAFI can guide engineers where to change the code while CryptoGuard only prints wrong pattern for some cases; 3) SAFI and CryptoGuard have very close cases number in some cases. As for running time comparison, SAFI is faster than CryptoGuard except for one case \emph{flume-file-channel-1.9.0.jar}. The reason is that the slowest part of our process is to build the callgraph and the backward slicing. We use the Wala built-in functions. Although we have optimized the speed of building the callgraph and prune the callgraph, it is still slower than the CryptoGuard. Moreover, due to the callgraph generation, in some cases, the callgraph is not well reflected in the original code architecture. However, the other parts run fast. Based on our experiment, the actual security-related data-flow analysis takes less than two seconds among these 13 projects. In our future work, we will improve the callgraph and implement the security-related slicing to increase the speed further so that SAFI can give the suggestion in real-time. 



\begin{table*}[h]
    \centering
    \begin{tabular}{c|c|c|c|c}
        Category & Total Case\# & Correct Case \#  & SAFI Detected \# & SAFI Gave Fix \# \\
        \hline
        brokencrypto & 36 & 1 & 35 & 35\\
        \hline
        brokenhash & 28 & 1 &27 & 27\\
        \hline
        dummycertvalidation & 3 & 0 & 3 & 1 \\
        \hline
        dummyhostnameverifier & 4& 1 &3 &3\\
        \hline
        ecbcrypto & 8 & 1 &7 &5\\
        \hline
        http &9 &2 &9 &9\\
        \hline
        impropersslsocketfactory &4 &0 &4 &4\\
        \hline
        insecureasymmetriccrypto & 6 &1 &5 &3\\
        \hline
        pbeiteration &9 &1 &8 &8\\
        \hline
        predictablecryptographickey &10 &1 &9 &9\\
        \hline
        predictablepbepassword &11 &1 &10 &10\\
        \hline
        predictableSeeds & 17 &1 &16 &16\\
        \hline
        staticinitializationvector & 10 &1 &9 &9\\
        \hline
        staticsalts &9 &1 &8 &8\\
        \hline
        untrustedprng &2 &1 & 1 & 1\\
    \end{tabular}
    \caption{CryptoBench Result}
    \label{tab:cryptoBench}
\end{table*}

\begin{table*}[hbtp]
    \centering
    \begin{tabular}{c|c|c|c}
        Filename &  SAFI Running Time (s) & CryptoGuard Runtime(s) & File Size (KB)\\
        \hline
        apacheds-kerberos-codec-2.0.0.AM25.jar & 5.34 & 8.85 & 672\\
        \hline
        artemis-commons-2.11.0.jar & 4.58 & 6.31 & 360\\
        \hline
        deltaspike-core-impl-1.9.2.jar & 2.65 & 3.61 & 206\\
        \hline
        flume-file-channel-1.9.0.jar& 142.91 & 5.5 & 294\\
        \hline
        hadoop-hdfs-3.2.1.jar & 15.78 & 70.68 & 5820\\
        \hline
        jclouds-core-2.2.0.jar & 5.87 & 8.92 & 906\\
        \hline
        %shindig-common-3.0.0-beta4.jar & 3.51 & 4.12 & 311 \\
        % \hline
        shiro-crypto-cipher-1.5.0.jar & 2.02 & 1.85 & 24\\
        \hline
        wagon-provider-api-3.3.4.jar & 2.10 & 1.95 & 55\\
        \hline
        wss4j-ws-security-common-2.2.4.jar & 4.24 & 7.74 & 330\\
        \hline
        wss4j-ws-security-stax-2.2.4.jar & 2.25 & 6.67 & 400\\
        \hline
    \end{tabular}
    \caption{10 Apache Project Running Time Comparison}
    \label{tab:Apache Running Time}
\end{table*}


% corrected the table not include different rule. change the domian knowlwdge.  F1 score report  % crpto match with our rule. 

\begin{table*}[hbtp]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c}
        Filename &  \makecell{SAFI\\Found\\Cases (s)} & \makecell{CryptoGuard\\Found\\Cases} & \makecell{Human\\Inspection\\Cases} & \makecell{Precision \\ SAFI/Cryptoguard} & \makecell{Recall \\SAFI/CryptoGuard} & \makecell{F1 score \\ SAFI/Cryptoguard} \\
        \hline
        apacheds-kerberos-codec-2.0.0.AM25.jar & 21 & 5 & 10 & 1/1 & 1/0.5 & 1/0.67\\
        \hline
        artemis-commons-2.11.0.jar & 6 & 6 & 3 & 1/1 & 1/1 & 1/1\\
        \hline
        deltaspike-core-impl-1.9.2.jar & 1 & 1 & 1& 1/1 & 1/1 & 1/1\\
        \hline
        flume-file-channel-1.9.0.jar & 2 & 2 & 1 & 1/1 & 1/1 & 1/1\\
        \hline
        hadoop-hdfs-3.2.1.jar & 5 & 5 & 5 & 1/1 & 1/1 & 1/1\\
        \hline
        jclouds-core-2.2.0.jar & 6 & 5 & 2 & 1/1 & 1/1 & 1/1\\
        % \hline
        % shindig-common-3.0.0-beta4.jar & 2 & 3 & 2 & 1/1 & 0\\
        \hline
        shiro-crypto-cipher-1.5.0.jar & 2 & 1 & 0 & N/A & N/A & N/A\\
        \hline
        wagon-provider-api-3.3.4.jar & 1 & 1 & 0 &  N/A& N/A & N/A\\  
        \hline
        wss4j-ws-security-common-2.2.4.jar & 5 & 4 & 5 & 1/1 & 1/0.8 & 1/0.89\\
        \hline
        wss4j-ws-security-stax-2.2.4.jar &5 & 1 & 5 & 1/1 & 1/0.2 & 1/0.33\\
        \hline
    \end{tabular}}
    \caption{10 Apache Project Result Comparison}
    \label{tab:Apache Result}
\end{table*}

In summary, SAFI can generate the pattern and detect the common vulnerable cases at a speed that not slower than state-of-the-art. 

==> Result/EvaluationRQ2.tex <==
%  2. effective of the tool, real work project. 100 projects. 
\subsection{RQ2: How does SAFI perform on 100 Apache projects?}

To further study the performance and invulnerability against the real project, from Github, we download the top 100 project source codes that satisfy the following criteria:
\begin{itemize}
    \item It must be the Apache project.
    \item It has the crypto API calls.
\end{itemize}

% no experinece 
% professional check

We compiled the top 100 Apache projects sorted by stars. After compilation, the total number of jar files is 3578 since it contains the dependencies of projects. We use SAFI to check all these jar files, and the result is shown in Table~\ref{tab:100 projects}.

% {'Rule Cipher getInstance': 23,
%  'Rule IvParameterSpec <init>': 9,
%  'Rule KeyPairGenerator initialize': 0,
%  'Rule KeyStore load': 31,
%  'Rule MessageDigest getInstance': 116,
%  'Rule PBEKeySpec <init>': 9,
%  'Rule PBEParameterSpec <init>': 8,
%  'Rule Random <init>': 420,
%  'Rule SecretKeySpec <init>': 25,
%  'Rule SecureRandom setSeed': 0}

% show that in some case, the api is used in vulnerable but left in purpose or not for the security purpose

From Table~\ref{tab:100 projects}, SAFI found a lot of security issues in the Apache project. However, when we check the occurrence of the insecure code snippets, we find:
\begin{itemize}
    \item \textbf{A lot of insecure code is written in the unit test code.} For the simplicity of writing the unit test code, engineers will not focus if the code is secure. Since the testing code will not run in the production environment, and if it is insecure, it will not have the security issue. When we study the RQ3, we have manually filtered out all this testing code when we push the change.
    \item \textbf{TrustAllManager is common on the project.} In some scenarios, engineers have to trust all incoming connections. Hence they wrote a specific class named \emph{TrustAllManager}. In this case, SAFI will warn the user that this is not secure, but further actions need to be done by engineers, such as leave a comment to warn other engineers that this class is not secure.
    \item \textbf{Insecure crypto APIs are used for other purposes.} Generally, engineers need to verify the file integrity. They will use \emph{MessageDigest.getInstance(``MD5")} or ``SHA-1" in the code. Under this circumstance, the code will not have any security concern, although MD5 and SHA-1 are vulnerable to the collision attack. But if engineers use SHA-1 or MD5 to encrypt the password, it will be dangerous since the length of a password is much less than the file size typically.  
\end{itemize}

For the second and the third findings, SAFI cannot handle the scenario correctly because SAFI can only examine the code by its type and name. It cannot read the purpose of engineers to write the code. Hence, the result might have a lot of noise for the users. In the future, we will let SAFI more intelligent in catching the hidden security problem.  

==> Result/EvaluationRQ3.tex <==
%  3. evaluation fix patch, accpted, mannuly detected
\subsection{RQ3: How does the fix patch work in practical projects?}

To find out if SAFI is helpful, we submit 65 pull requests using SAFI suggestion to   Apache projects. We notice that in the unit test, some programs intentionally leave a "TrustAll" function that accepts all SSL connections without any certification. We have filtered out all these cases when pushing the merge requests. The result is shown at Table~\ref{tab:PR}:

% feedback mistual postive netural. pass the unit test. response, pass 
% mainly report  maintain project  
% follow up question. , user student statiscti. accept. positive quto the response.  

\begin{table}[hbtp]
    \centering
    \begin{tabular}{c|c}
        Status &  Total \# \\  
        \hline
        Merge & 3 \\
        \hline
        Positive Feedback (exclude merge) & 1 \\
        \hline
        Unit Test Passed & 14 \\
        \hline
        Negative feedback & 7 \\
        \hline
        No Feedback (without archived project) & 12 \\
        \hline
        Unit Test Failed & 12 \\
        \hline
        Others & 10 \\
        \hline
        TOTAL & 60
    \end{tabular}
    \caption{Vulnerability Detection}
    \label{tab:PR}
\end{table}

\begin{table*}[hbtp]
    \centering
    \begin{tabular}{c|c|c|c}
        Apache Project Name & Stars & Merge Link & Comments \\  
        \hline
        apache/pulsar & 5.4k & https://github.com/apache/pulsar/pull/6447 &  \\
        \hline
        apache/beam & 3.8k & https://github.com/apache/beam/pull/11008 & Merged by \#10055 \\
        \hline
        apache/servicecomb-java-chassis & 1.6k & https://github.com/apache/servicecomb-java-chassis/pull/1604 & \\
        \hline
    \end{tabular}
    \caption{Apache Merge Project}
    \label{tab:Merge}
\end{table*}


Note that Apache projects have more strict about accepting the merge request outside the core developer. Our fix suggestions are been merged by three high stars (5.4k, 3.8k and 1.6k) Apache projects. 

For the positive side, three project owners have merged the code. For the high stars projects, the project owner quickly replied our request and merge the request. And for eight projects, we pass the unit tests. 

For the negative feedback, some developers leave responses that for speed consideration, they won't change the current encryption algorithm. Meanwhile, they have also implemented some other codes based on a specific algorithm. If the current encryption algorithm changes, they need to make more consequence change, which might be risky for them. A few developers are not happy with our commit message since we did not elaborate on the reason why we change.  

For the unit test failed, we manually inspect the error message generated from the Continuous Integration(CI). It can be broken down in the following reason:
\begin{enumerate}
    \item CI did not allow external push. 
    \item CI machine is down.
    \item The java code formatting is wrong.
\end{enumerate}

Like others, some projects had archived in Github, while some projects did not accept merges on Github, etc.

In summary, SAFI can help the engineer to detect the insecure code snippets. In some cases, it will fail to tell if the crypto API is used for security purposes. 





==> Result/limitation.tex <==
\section{Threat To Validity}

In this section, we discuss the threats to validity. There are a few limitations to our tools: 
\begin{enumerate}
    \item \textbf{Focus on the Java application only.} SAFI can only detect the security-related API on Java application. For Android API, it has some different crypto API than Java. Besides, for the misuse in Javascript, SAFI cannot detect it. To detecting the crypto API misuse in the Android application, users can add the template to the JSON file and specify the entry point of the application. As Javascript, SAFI needs to make some changes to handle the different IR in javascript. 
    \item \textbf{Generating the callgraph and slicing can be slow.} As we mentioned before, based on our experiment, Wala built-in callgraph and the built-in static slicing function can be slow since the callgraph can be complicated. Besides, the static slicing algorithm will give an approximate result that the result might not be accurate in some cases. In the future, we will implement a callgraph and slicing algorithm that only focuses on the security-related code to shrink the size of the callgraph.
    \item \textbf{The fix suggestion is not taken consideration of the purpose of the code.} As we run our tool on the practical projects, we found that the vulnerable code is in a) the unit test code; b) left in purpose. For instance, the engineer will leave the code to trust all connections in SSL in the unit test. And the engineer will use the ``SHA-1" or "MD5" for the file validation. Although it is not a security-related code, they use the crypto API. For SAFI, it cannot tell if the engineer uses the crypto API for security purposes. For solving the report in the unit test, engineers can filter the result generated by SAFI to get rid of the testing code. For the second case, it needs to manually decide if the suggested fix is suitable for the current scenarios. 
    
\end{enumerate}
    


